Active Human Pose Estimation via an Autonomous UAV Agent

One of the core activities of an active observer involves moving to secure a "better" view of the scene, where the definition of "better" is task-dependent. This paper focuses on the task of human pose estimation from videos capturing a person's activity. Self-occlusions within the scene can complicate or even prevent accurate human pose estimation. To address this, relocating the camera to a new vantage point is necessary to clarify the view, thereby improving 2D human pose estimation. This paper formalizes the process of achieving an improved viewpoint. Our proposed solution to this challenge comprises three main components: a NeRF-based Drone-View Data Generation Framework, an On-Drone Network for Camera View Error Estimation, and a Combined Planner for devising a feasible motion plan to reposition the camera based on the predicted errors for camera views. The Data Generation Framework utilizes NeRF-based methods to generate a comprehensive dataset of human poses and activities, enhancing the drone's adaptability in various scenarios. The Camera View Error Estimation Network is designed to evaluate the current human pose and identify the most promising next viewing angles for the drone, ensuring a reliable and precise pose estimation from those angles. Finally, the combined planner incorporates these angles while considering the drone's physical and environmental limitations, employing efficient algorithms to navigate safe and effective flight paths. This system represents a significant advancement in active 2D human pose estimation for an autonomous UAV agent, offering substantial potential for applications in aerial cinematography by improving the performance of autonomous human pose estimation and maintaining the operational safety and efficiency of UAVs.

==> preamble.tex <==
%
% --- inline annotations
%
\usepackage[dvipsnames]{xcolor}
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
% --- disable by uncommenting  
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}



==> sec/0_abstract.tex <==
\begin{abstract}
One of the fundamental activities of an active observer is to move in order to
obtain a “better” view of the scene. The definition of “better” however is dependent
on the task under consideration. In this paper, we consider the task of estimating the
pose of a human, given a video of the human’s activity. It may happen that the scene
(the acting human) has self-occlusions making it difficult or impossible to estimate
the human pose. In such a case, we will need to move the camera into a new
location in order to disambiguate, i.e. we need to obtain a “better” view of the scene.
The paper formalizes this ability.
Our proposed system for solving this problem consists of three components: a
NeRF-based Drone-View Data Generation Framework, an On-Drone Network for
Viewing Angle Estimation, and a Combined Planner for a Feasible Motion Plan that
will move the camera to a better position. The Data Generation Framework
employs NeRF-based techniques to capture a wide range of human poses and
actions, thus enriching the UAV’s capability in diverse scenarios. The Viewing Angle
Estimation Network is specifically engineered to assess current human poses and
compute optimal viewing angles for the UAV, ensuring a rapid and precise response
to the subject’s movements. Lastly, the Feasible Motion Plan integrates these
viewing angles with the UAV’s physical and environmental constraints, utilizing
efficient algorithms for safe and efficient flight paths.
The proposed system not only advances 2D Human Pose Estimation techniques but
also holds significant potential for practical applications in aerial cinematography,
enhancing the visual quality while maintaining UAV operational safety and efficiency.
% The system is comprehensively tested in many simulation environments.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Recent advancements in aerial robotic technologies have significantly improved the use and abilities of aerial robots in many industries. \cite{stocker2017review, nex2014uav, baiocchi2013uav}. A key aspect of modern aerial robots is their ability to be equipped with video capture sensors, such as cameras, transforming them into dynamic platforms for aerial videography \cite{zhou2022swarm}. The mobility and agility of aerial robots make them highly effective for aerial cinematography, allowing for versatile footage capture from optimal angles with minimal equipment. The growing demand in entertainment, industrial, and military sectors has shifted aerial cinematography's focus from static objects to dynamic human subjects and the technical challenge is how to autonomously adjust drone's viewing direction in order to best viewing human subject while doing navigation. 

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/challenge_view.PNG}
    \caption{UAV's viewing angles of a human subject is more than only 360 degree but actually in a hemisphere-like space }
    \label{fig:challenge_view}
\end{figure}

Specifically, the challenges of achieving this autonomous viewing-direction adjustment for UAV pose estimation can be summarized as follows: 1) What is the criterion for adjusting UAV's viewing direction when inspecting human? 2) How to get the guidance when UAV is  

% Specifically, the challenges of achieving this autonomous viewing-direction adjustment for UAV pose estimation can be summarized as follows: 1) Acquisition of Comprehensive UAV View Data: This task is not limited to conventional 360-degree views but extends to a hemispherical viewing space, as depicted in Fig. \ref{fig:challenge_view}. Such comprehensive coverage requires a UAV to capture a multitude of angles, both horizontally and vertically, ensuring no potential occlusions in the line of sight. This extensive data collection demands advanced UAV navigation systems capable of intricate maneuvering and positioning.  2) Predictive Analysis for Optimal Viewing Angles: This requires a sophisticated understanding of human anatomy and movement patterns, coupled with advanced computational models that can process current pose data and predict future states. The objective is to foresee which angles will most effectively mitigate occlusions and provide the clearest view of the subject. 3) Strategic Selection of Feasible Viewing Angles: by selecting a subset of the optimal viewing angles that are not only theoretically ideal but also practically executable by a UAV. This selection must consider the UAV's physical and operational limitations, such as its flight dynamics, battery life, and the ability to rapidly change positions. Furthermore, environmental factors, including wind patterns and physical obstructions, must be accounted for to ensure safe and effective UAV operation. The development of a decision-making framework that integrates these considerations is crucial for the practical implementation of UAV-based human pose estimation.  

\begin{figure*}[t]
    \centering
    \includegraphics[width=0.9\textwidth]{Figures/teaser.pdf}
    \caption{The Illustration of the problem we are trying to solve and our proposed approach. As upper row shows, the 2D human pose estimation is a easy problem if the camera viewing angle is picked carefully otherwise it may not be solvable due to self-pose or environmental occlusions. Our proposed approach is an integrated system consists of 1) Drone-view Data Synthesis, 2) a learned network to "lookup" 3D perception guidance field for better viewing angle selection guidance for th drone, and 3) a combined planner combines both traditional navigation cost maps and inferred 3D perception guidance field to achieve joint motion plan for collision avoidance navigation and selecting good viewing-angle for human pose estimation.    }
    \label{fig:teaser}
\end{figure*}

To address the challenges posed by dynamic videography using UAVs, we propose a sophisticated, integrated autonomous UAV videography system, as illustrated in Fig. \ref{fig:teaser}. This system is engineered to intelligently interpret human poses and proactively reposition itself to capture optimal visual content. The architecture of this system can be delineated into three primary components: 1) Drone-View Human Subject Data Generation Framework: This framework is designed to capture a wide array of human poses and actions, under varying environmental perspectives. By utilizing advanced vision techniques(HumanNerf) \cite{weng_humannerf_2022_cvpr}, this framework will enable the UAV to have a profound understanding of human subjects in different scenarios, enhancing its ability to adapt to real-world videography tasks, 2) Robust and Efficient On-Drone Network for Viewing Angle Estimation: This network is tailored to analyze the current human pose and swiftly compute the best subset of next viewing angles, which aims to process complex visual inputs in real-time, ensuring that the UAV can react promptly and accurately to dynamic subjects. The efficiency of this network is crucial, as it directly impacts the UAV's ability to operate under computational and power constraints typically associated with autonomous drones, 3) Combined Planner for Feasible Motion Plan: our proposed system is a sophisticated planning module that combines the network's viewing angle recommendations with the UAV's kinodynamic and environmental constraints. This combined planner employs advanced algorithms to chart a feasible motion plan that not only adheres to the suggested viewing angles but also respects the physical limitations of the UAV and navigational challenges posed by the environment. By integrating this planner, the UAV can maneuver in complex environments with agility and precision, ensuring high-quality videography while maintaining safety and operational efficiency.

We will elaborate on the specific details and analysis of drone-viewing data generation in the next section. For the on-drone network part,to ensure the real-time performance of the system, the input to the network will be a 2D human skeleton sequence estimated by OpenPose \cite{OpenPose}. The output is the error vector of 2D human pose estimation at all set viewpoints (we call it 3D perception guidance field). We designed a very lightweight network to learn the relationship between the best subset of next viewing angles and the current human pose estimation by training it on our generated dataset. The estimation of the 3D perception guidance field does not need to be very accurate, but it needs to provide enough clues for subsequent motion planning. 
For motion planning part, based on \cite{Zhou2020EGOPlannerAE} and \cite{wang2022gpa}, we developed a perception-aware motion planning framework that can not only follow the best viewpoint, but also be able to generate smooth trajectory, avoid the occolusion between the target and the Uav and ensure the flight safety.

Therefore, our contribution can be concluded as:
\begin{itemize}
    \item A drone-view data generation framework for different human poses 
    \item A Robust and efficient on-drone network for the best subset of next viewing angles estimation based on the current human pose
    \item A combined planner that coordinates the perspective-aware guidance from network and traditional drone's navigation constraints to a feasible motion plan for improving 2D HPE, a computer vision task.
\end{itemize}

We make our entire system totally integrated so that all the above three parts interact with each other and can be applied to real-world scenarios.

% %-------------------------------------------------------------------------
% \subsection{Language}

% All manuscripts must be in English.

% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}


==> sec/2_formatting.tex <==
\section{Related Works}
\label{sec:formatting}

(1. Paragraph: On Drone Aerial Cinematography) 

(2. Paragraph: On 2D Human Pose Estimation) 

(3. Paragraph; On NeRF and Human NeRF)

% The recent progress in Computer Vision and Motion Planning has greatly enhanced the capabilities of Unmanned Aerial Vehicles (UAVs), particularly in the context of tracking and filming human subjects \cite{autofilmer, elastictracker, intergratedmotionplanner, learnedartisticdecision-makings}. These advancements have been significant, allowing UAVs to autonomously navigate and adjust their filming angles and positions. However, most of these developments have been centered around what can be termed as "low-level autonomy". This refers to the UAVs' ability to autonomously execute motion planning based on predefined waypoints or viewing directions. In these scenarios, the high-level task, which involves more complex decision-making and subjective judgment, remains quite rudimentary. For instance, UAVs have been used to follow target human subjects or to carry out artistic filming based on human input. Some previous works have usefully explored this application scenario. Zhang et al. proposed an autonomous aerial camera system (Auto Filmer) \cite{autofilmer} integrating customized shots and UAV dynamics. The system includes a user-friendly interface for real-time shot creation, a kinematic path search process for safe shooting paths, and joint optimization for trajectory generation. Their work presents extensive simulations and real-world experiments that validate the effectiveness of their approach. Experimental content includes tracking video in complex environments, shooting in dense environments, paper airplane tracking, etc. Their results show that their system is capable of stable shooting without a tilting gimbal and can continuously shoot moving targets in cluttered environments while avoiding obstacles. This type of usage, while beneficial, doesn't fully exploit the potential of UAVs in more advanced and high-level tasks.


% One key area that remains underexplored is the use of UAVs' mobility and dynamic camera angles in enhancing fundamental computer vision tasks. A significant question arises: Can we leverage the flexibility and dynamic viewing capabilities of UAVs to improve crucial tasks like human pose estimation? Traditional methods of human pose estimation are often limited by static camera angles and positions. UAVs, with their ability to move freely and adjust their filming perspectives, could potentially provide more comprehensive and varied visual data. This, in turn, could lead to more accurate and detailed analysis in computer vision applications, such as improving the algorithms for pose estimation. The challenge lies in developing more sophisticated algorithms and systems that can not only handle the complex motion planning and control of UAVs but also integrate this with advanced computer vision techniques to truly revolutionize how we capture and interpret visual data of human subjects.

% The pursuit of enhanced Human Pose Estimation (HPE) methodologies is pivotal in advancing the field of human-centric computer vision applications \cite{andriluka20142d, chen20173d}, particularly in robotics and human activity recognition systems. The main endeavor lies in the development of robust and efficient HPE algorithms that can effectively interpret and analyze human posture and movement. Among the various models employed for this purpose, OpenPose \cite{OpenPose} has emerged as a standard in 2D HPE, especially in robotics research and industrial applications. This model is renowned for its robustness and optimized performance on computational platforms such as the NVIDIA Jetson series, which are tailored for robotic applications. However, despite the remarkable capabilities of OpenPose \cite{OpenPose}, it exhibits limitations in handling certain human pose cases, as illustrated in Fig.\ref{fig:teaser}. The primary challenge stems from the self-occlusion of body parts, a phenomenon that occurs when certain angles of camera viewing obscure parts of the human body, thus impeding the model's ability to accurately detect human joints and skeletal structure. This limitation is not just a trait of OpenPose \cite{OpenPose} but is indicative of a broader issue in 2D HPE methodologies.

% A critical observation in this regard is that when there is an absence of occlusion, both environmental and self-induced, standard methods like OpenPose \cite{OpenPose} demonstrate robustness and accuracy in 2D HPE. However, in scenarios where occlusion is present, these methods struggle, resulting in inaccurate or missing detections of human joints and skeletal structures. This challenge predominantly arises due to insufficient visual information available from certain camera angles to infer the occluded body parts. Such a predicament suggests that the issue at hand transcends mere improvements in vision models; it is not solely a "vision" problem that can be rectified with enhanced visual data processing techniques.

% In light of this understanding, an innovative approach is proposed to circumvent the challenges posed by occlusions. The strategy involves utilizing the mobility of UAVs to autonomously adjust the viewing direction of the subject, thereby mitigating the issue of occlusions. By ensuring that the camera angles are optimized to avoid situations where body parts are occluded, the data fed into HPE models like OpenPose \cite{OpenPose} is devoid of the 'ill-posed' attributes that typically hinder accurate pose estimation. Consequently, this approach aims to provide 'cleaner' and more informative data to standard HPE methods, thereby enhancing the robustness and accuracy of 2D human pose estimation in UAV-based applications. This solution underscores a shift from a purely computational approach to an integrated methodology that combines advanced vision modeling with strategic maneuvering of observational platforms.


==> sec/3_finalcopy.tex <==
\section{Perception-aware motion planning}
 To bridge the gap between the perception and motion planning, we introduce our proposed perception-aware motion planning framework. In the proposed framework, the perception loss is added into the motion planning cost function as one of the costs. To achieve that, we built a differentiable distance field called Pose-enhanced Euclidean Distance Field. The construction of this field is described below.
 
 The output of Pose Estimation Error Predictor is a 2-D map $\mathcal{E}: \mathbb{R}^{m \times n} \rightarrow \mathbb{R}$, which can be expressed as $e(i, j) = \mathcal{E}_{i, j}$, for $i = 1,2,...,m$ and $j = 1,2,...,n$.

\begin{equation}
% \begin{aligned}
    J_{pose} = \lambda_p \sum_{i=0}^{M} c(p_i) p_i^1
% \end{aligned}
\end{equation}
where $p_i^1 = \frac{\partial \Xi(p_i)}{\partial p_i}$ can be efficiently acquired from P-ESDF, and $c(p_i)$ can be expressed as:
\begin{equation}
% \begin{aligned}
    c(p_i) = \left\{ 
    \begin{aligned}
            \frac{1}{2\rho}(\Xi(p_i)-\rho)^2, \Xi(p_i) \leq \rho\\
            0, \Xi(p_i) > \rho
    \end{aligned}
    \right.
% \end{aligned}
\end{equation}

The result is shown in Fig. \ref{fig:esdf}.

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{Figures/esdf.png}
    \caption{Visualization for the proposed distance field.}
    \label{fig:esdf}
\end{figure}

==> sec/Conclusion.tex <==
\section{Conclusion}

Overall, we proposed a novel methodological framework focusing particularly on the dynamic and accurate human pose estimation. This comprehensive system comprises three interconnected components, each playing a pivotal role in enhancing the efficacy and applicability of the UAV in complex videography settings. 1) Drone-View Data Generation Framework: This component is designed to capture an extensive range of human poses and actions. By utilizing advanced vision techniques, this framework provides a rich dataset, enabling the UAV to adapt to a wide variety of filming conditions. This diversity in data is crucial for the system to handle real-world scenarios with varying degrees of complexity and dynamism. 2) On-Drone Network for Viewing Angle Estimation: it utilize to analyze the current human pose and, based on this analysis, computes the most effective subset of next viewing angles. This network is a testament to the integration of advanced machine learning techniques with UAV technology, resulting in a system capable of making real-time, informed decisions about camera positioning and movement. 3) Combined Planner for Feasible Motion Plan: The final component is a comprehensive planner that melds the insights gained from the network with traditional drone navigation constraints. It ensures that the motion of the UAV is not only optimal for capturing the desired imagery but also adheres to safety and feasibility standards. The culmination of these components results in a method that is not only innovative but also practical for real-world applications. Our system offers a versatile solution for UAV cinematography that can adapt to varying environmental conditions and subject dynamics. Finally, our system is comprehensively evaluated in various challenging environments.

==> sec/Data_Generation.tex <==
\section{Drone-View Data Generation}
In the preceding discussion, as delineated in Fig.\ref{fig:challenge_view}, the acquisition of data for drone-view perspectives of human subjects necessitates the simulation of varying viewing angles within a hemispherical space. To the best of our current knowledge, a dataset encompassing such parameters is not yet extant. Typically, this type of data can be procured through one of three methodologies: 1) Utilizing Unmanned Aerial Vehicles (UAVs) to capture imagery of various human subjects from multiple angles, 2) Constructing a comprehensive array of cameras capable of covering the hemispherical space, or 3) Employing simulation software such as Blender or Unity to generate projected image views from human models. However, each of these methods presents distinct challenges and practical difficulties, particularly in the context of a course project. The use of UAVs or camera arrays to collect a dataset that meets our standards is an exceedingly time-intensive endeavor. Moreover, datasets captured in simulated environments are likely to exhibit a domain gap when compared to real-world scenarios, potentially hindering the generalizability of models trained on such data in actual situations. The advantages and disadvantages of these diverse methods for generating drone-view data are further explicated in Table. \ref{table:data}.


In our research, we identified a novel free-viewpoint rendering method, known as HumanNeRF \cite{weng_humannerf_2022_cvpr}, which demonstrates significant utility in scenarios involving complex human body movements, aligning seamlessly with our data generation prerequisites. This technique is capable of rendering 360-degree novel viewpoints for any frame within a given input video. Our approach involves collecting images within a specified hemispherical space in a 3D scene rendered by HumanNeRF \cite{weng_humannerf_2022_cvpr}. These images will then be processed through the OpenPose \cite{OpenPose} pipeline to derive 2D human pose estimation sequences, serving as our primary input. By posing these estimations with the ground truth data extracted from the 3D rendered scene, we aim to ascertain the discrepancies in human pose estimation from various viewpoints. This will facilitate the construction of a 3D perception guidance field, a novel concept in our research. The detailed process for generating this 3D perception guidance field is illustrated in Fig.\ref{fig:data_gen}.
\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{Figures/nerf_pair_data.PNG}
    \caption{Proposed NeRF-based 3D perception guidance field data generation process: For a give human and human pose, we will use the 2D annotation to perform batch triangulation and get 3D skeleton for that pose, in the meanwhile we will render the synthesized image for "drone views", finally we both reproject ground truth 3D skeleton on NeRF poses to get ground truth 2D keypoints and run OpenPose \cite{OpenPose} for predicted ones, in this way we can get the paired data of 2D observation and corresponding 3D perception guidance field. }
    \label{fig:data_gen}
\end{figure}


% \begin{table}[h]
% \caption{Table of Comparison of Different Drone-view Data Generation Methods}
% \label{table:data}
% \begin{tabular}{|c|cll|c|cl|}
% \hline
% \begin{tabular}[c]{@{}c@{}}Data\\ Generation \\ Methods\end{tabular} & \multicolumn{3}{c|}{Cost} & \begin{tabular}[c]{@{}c@{}}Viewing \\ Angle \\ Resolution\end{tabular} & \multicolumn{2}{c|}{\begin{tabular}[c]{@{}c@{}}Photo\\ Realistic?\end{tabular}} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Drone \\ Capture\end{tabular} & \multicolumn{3}{c|}{Medium} & Discrete & \multicolumn{2}{c|}{Yes} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Camera \\ Array\end{tabular} & \multicolumn{3}{c|}{High} & Discrete & \multicolumn{2}{c|}{Yes} \\ \hline
% \begin{tabular}[c]{@{}c@{}}Simulation\\ Software\end{tabular} & \multicolumn{3}{c|}{Low} & Discrete & \multicolumn{2}{c|}{No} \\ \hline
% Our & \multicolumn{3}{c|}{Low} & Continuous & \multicolumn{2}{c|}{Yes} \\ \hline
% \end{tabular}
% \end{table}



\begin{table}[t!]
    \centering
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{@{}cccc}
    \toprule
    \textbf{Method} & \textbf{Cost} & \textbf{Viewing Angle Resolution} & \textbf{Photo Realistic}   \\ 
        \midrule
        Drone Capture \cite{live} & Medium   & Discrete & \checkmark \\
        Camera Array \cite{live} & High  & Discrete & \checkmark \\
        Simulation Software \cite{live} & Low  & Discrete &  -- \\
        \toprule
         Ours & Low & Continuous & \checkmark \\
        \toprule
    \end{tabular}
    }
    \captionsetup{font=small}
    \caption{Table of Comparison of Different Drone-view Data Generation Methods}
    \label{tab:datasets}
\end{table}

==> sec/Experiments.tex <==
\section{Experimental Results}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{Figures/sim_large.pdf}
    \caption{Simulation environment. the upper row of each figure is images captured using the onboard camera, the bottom row indicates the third person view of the experiment. The 3D perception guidance field is represented as the semi-sphere field around the drone, different color indicates the quality of each view point, from green to red indicate the good to poor. The green arrow means the best viewpoint comprehensively consider the pose estimation accuracy, occlusion and flight safety. \textbf{(a - d): }The best viewpoint (green arrow) changes with regard to the change of the human pose, and the UAV follows the best view point in real-time.  \textbf{(e - h): }When there are both target and obstacles observed in the encironment, the UAV automatically choose the second best viewpoint to avoid the occlusion and ensure the safety.}
    \label{fig:sim}
\end{figure*}

\subsection{Implementation Details}
\label{sec:ImpleDetail}


\begin{figure}[hb]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/drone.pdf}
    \caption{Drone. Left: simulated drone. Right: real-world self-assembled drone.}
    \label{fig:drone}
\end{figure}

Our simulated and real-world aerial vehicle platform are shown in Fig. \ref{fig:drone}. 
The simulated vehicle is equipped with a Velodyne Puck Lidar used as the range sensor for navigation planning. For the real-world drone, a self-assembled flight platform with diameter 400mm, height 119mm and weight 1167g is chosen for demonstration. The perception module we use is Intel D435 depth camera, which outputs depth images for environment perception and stereo gray-scale images for localization and human-drone interaction simultaneously. A NVIDIA Xavier is mounted for computation.


The onboard autonomy system of the UAV integrates several key navigation modules from our development environment \cite{cao2022autonomous, zhang2014loam}. These include terrain analysis and waypoint following, which are based on kinodynamically feasible trajectories generated by the local planner. These components serve as fundamental navigation modules. Atop this system architecture, the proposed perception-aware planner operates, harnessing the capabilities of the underlying modules to enhance its navigational efficiency and effectiveness. This layered integration facilitates a robust and adaptive UAV operation, capable of intelligently responding to dynamic environmental factors and mission objectives


\subsection{Evaluation for On-drone Best View Point Generation}
\label{sec:EvaPerception}
To demonstrate the performance of the proposed On-drone Best View Point Generation method, we implement this experiment in challenging real-world scenarios as shown in Fig. \ref{fig:ResPercep}. 

In the depicted figure, the algorithm initially normalizes the estimated 2-D pose, as detailed in the methodology section. Subsequent to this normalization, a dense distance field, also referred to as an error map, is generated. Each point within this distance field represents the quality of pose estimation, as illustrated in Fig. \ref{fig:ResPercep}. Various colors are utilized to denote the quality of different viewpoints in relation to the subject. As the person moves, viewpoints located directly in front of the individual are assigned lower costs due to their optimal visibility. Conversely, viewpoints situated behind the person are typically associated with higher costs. This is because such angles are more likely to result in occlusions of critical features like the face and arms. The error map serves as a guiding mechanism for the UAV, directing it to capture the subject from viewpoints that incur the lowest cost, thus optimizing the quality of pose estimation and the overall effectiveness of the tracking process.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/ErrRes.pdf}
    \caption{The result for 3-D best viewpoint estimation.}
    \label{fig:ResPercep}
\end{figure}

\subsection{Evaluation for On-drone Perception-aware Motion Planning}
\label{sec:EvaPlanning}

To evaluate the efficacy of the On-drone Perception-aware Motion Planning method, we conducted an experimental implementation in complex, cluttered environments characterized by numerous obstacles, as depicted in Fig. \ref{fig:planenv}. 

In obstacle-free environments, the UAV consistently adheres to the optimal viewpoint. However, upon encountering obstacles, the UAV demonstrates the capability to maintain this optimal viewpoint while simultaneously navigating around these obstructions. In scenarios where obstacles are proximate or densely situated, the planning framework proactively shifts to the second-best viewpoint. This adjustment is crucial for mitigating occlusion issues between the target and the UAV, and for maintaining safety by avoiding obstacles. Upon successful navigation past these obstacles, and ensuring that there is no occlusion obstructing the view of the target, the UAV then seamlessly plans and executes a trajectory to return to the primary, most advantageous viewpoint. This dynamic adaptability in the UAV's path planning, particularly in challenging and cluttered environments, underscores the robustness and sophistication of the proposed On-drone Perception-aware Motion Planning method.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/plan_env.png}
    \caption{The testing environment for the proposed motion planning framework.}
    \label{fig:planenv}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.6\linewidth]{Figures/obs_avoid.pdf}
    \caption{Perception-aware motion planning experiment. \textbf{(a): }The UAV follows the best viewpoint (green arrow). \textbf{(b): }The UAV can still follow the best view point and avoid the obstacle at the mean time. \textbf{(c-d): }To avoid the occlusion between the target and the UAV, and also avoid the obstacles for safety, the proposed planning framework automatically switch to the second-best viewpoint. \textbf{(e-f): }After avoiding the obstacle, and there is no occlusion between the target and the UAV, the UAV plans a smooth trajectory to go back to the best viewpoint.}
    \label{fig:ObsAvoid}
\end{figure}


\subsection{System-level Experiment}
\label{sec:SysExp}
To validate the robustness and overall performance of our integrated system, we conducted an experiment in a realistically challenging, cluttered environment with numerous obstacles using Unity, as illustrated in Fig. \ref{fig:sim}. This experiment was designed to replicate complex real-world conditions. The perception aspects were simulated within Unity, while the control and motion planning components were simulated in ROS \cite{Quigley2009ROSAO} with Rviz \cite{094f52e6f6804ec09c1b4e0b4f96a445} employed for visual representation.

As indicated in Fig. \ref{fig:sim}, the optimal viewpoint (represented by a green arrow) dynamically adjusts in response to changes in the human subject's pose. The UAV is programmed to track and align with this best viewpoint in real-time, showcasing its responsiveness to the target's movements. In scenarios where both the target and obstacles are present within the UAV's operational environment, the system intelligently opts for the second-best viewpoint. This strategic choice is critical for avoiding visual occlusion between the UAV and the target, and for ensuring safety by steering clear of obstacles. This approach effectively demonstrates the system's capability to adapt to varying environmental conditions while maintaining high-quality perception and safe navigation.

==> sec/visionNet.tex <==
\section{Mapping 2D Observation to 3D perception guidance field}
In the realm of autonomous drone navigation, the deployment of a perception guidance system utilizing NeRF-synthesized 'Drone-view' data pairs necessitates the creation of a specialized lookup table. This table is pivotal for referencing human image and 3D perception guidance field pairs, and it must be capable of interpolating between pre-computed training data points to accommodate real-world scenarios. Several paramount considerations guide the design of this lookup table:
\begin{itemize}
    \item Interpolation and Lookup Capability: The table must efficiently interpolate between existing data points, ensuring accurate representation of human images and 3D perception guidance field. This is essential for handling the dynamic and diverse scenarios encountered in real-world applications.
    \item Robustness to Drone-Specific Characteristics: The system should be inherently robust to various challenges specific to drone operation, including: 1) Scale Variability: It must account for size variations arising from different human subjects or alterations in the drone-to-human distance, 2) Camera Translation: Given the drone's mobility, the system should be adept at handling changes in the camera's position, 3) Rotational Adjustments: It should also be resilient to rotations along the camera's optical axis, a common occurrence due to drone vibrations during flight. 
    \item On-Drone Computational Efficiency: Considering the limited processing capabilities of drones, which simultaneously manage vision tasks and maintain balance and pose estimation, the lookup table must be computationally lightweight. This ensures minimal consumption of the drone’s computational resources.
\end{itemize}

To address these considerations, a simplified auto-encoder network is employed for visual guidance, as depicted in Fig. \ref{fig:method}. This network architecture is characterized by a minimal number of weights, enhancing its efficiency. Through input abstraction and normalization processes, the system demonstrates a negligible simulation-to-reality gap and robustness against changes in scale, translation, and rotation. This is further evidenced in real-world application scenarios, as shown in Fig. \ref{fig:ResPercep}.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{Figures/method.pdf}
    \caption{Proposed PoseErrNet: It consists with two major parts, 1) Input abstraction and normalization to deal with the sim-to-real gap and scale, translation, rotation invariance for the drone applications, 2) The auto-encoder network and output space abstraction to map from normalized 2D observation to 3D perception guidance field}
    \label{fig:method}
\end{figure*}

